Optimal and Approximation Algorithms for Joint Routing and Scheduling in Millimeter-Wave Cellular Networks

Millimeter-wave (mmWave) communication is a promising technology to cope with the exponential increase in 5G data traffic. Such networks typically require a very dense deployment of base stations. A subset of those, so-called macro base stations, feature high-bandwidth connection to the core network, while relay base stations are connected wirelessly. To reduce cost and increase flexibility, wireless backhauling is needed to connect both macro to relay as well as relay to relay base stations. The characteristics of mmWave communication mandates new paradigms for routing and scheduling. The paper investigates scheduling algorithms under different interference models. To showcase the scheduling methods, we study the maximum throughput fair scheduling problem. Yet the proposed algorithms can be easily extended to other problems. For a full-duplex network under the no interference model, we propose an efficient polynomial-time scheduling method, the {\em schedule-oriented optimization}. Further, we prove that the problem is NP-hard if we assume pairwise link interference model or half-duplex radios. Fractional weighted coloring based approximation algorithms are proposed for these NP-hard cases. Moreover, the approximation algorithm parallel data stream scheduling is proposed for the case of half-duplex network under the no interference model. It has better approximation ratio than the fractional weighted coloring based algorithms and even attains the optimal solution for the special case of uniform orthogonal backhaul networks.

==> fd-approx-algo.tex <==
\section{Approximation Algorithm for Full-Duplex Maximum Throughput Fair Scheduling}
\label{s:fd-approx-algo}

In \S \ref{s:fd-sched-fair}, we have proposed an optimal polynomial-time algorithm for the FD-MTFS problem. Although being optimal, it may incur a high execution time, especially when the number of nodes or of RF chains is large. Hence, we will propose a runtime efficient {\em edge-coloring based approximation} (EC) algorithm that has a provable worst-case max-min throughput. It follows a two-step approach: (i) computing the link time and (ii) edge-coloring based scheduling.

\subsection{Step (i): Computing Link Time}
To compute the link time exactly, we need to include the constraints for the schedule polytope~\eqref{eq:link-active-time}. To reduce the execution time, instead we consider only a small set of constraints that are necessary but not sufficient for a feasible unit time schedule. 
The linear program for computing an upper bound of the max-min throughput is 
\begin{IEEEeqnarray}{lrClr}
\IEEEyesnumber \IEEEyessubnumber*
  \textnormal{max} & \theta & & & \\
  \textnormal{s.t. } &\sum_{e\in\delta_D^-(v)} c(e) t_e
  -\sum_{e\in\delta_D^+(v)}c(e) t_e& \ge & \theta
  \quad\forall\,v\in M(D)\IEEEeqnarraynumspace \label{eq:ec-step1-theta}
  \\
  & \sum_{e \in \delta_D(v)} t_e & \le & r(v) \quad \forall \, v \in V(D) \IEEEeqnarraynumspace \label{eq:ec-step1-node} \\
  &  t_e & \ge & 0 \quad \forall \, e \in E(D) \IEEEeqnarraynumspace \label{eq:ec-step1-link}
\end{IEEEeqnarray}
where $\delta_D^-(v)$, $\delta_D^+(v)$ and $\delta_D(v)$ are the set of links in $D$ that enter vertex $v$, leave $v$ and are incident to $v$, respectively. $t_e$ is the link time of the arc $e$. 
\eqref{eq:ec-step1-theta} signifies that the throughput at each relay BS is at least $\theta$.
\eqref{eq:ec-step1-node} is necessary because the links incident to $v$ can be scheduled by at most $r(v)$ number of RF chains simultaneously. 

With the solution $\theta$, we go on to compute the link time for the maximum network throughput:
\begin{IEEEeqnarray}{lC}
\label{eq:ec-step1-tput}
  \textnormal{max} &\sum_{\mathclap{e \in \{\delta_D^+(v) | v \in B(D) \}}} c(e) t_e
  \nonumber\\
  \textnormal{s.t.}&\textnormal{\eqref{eq:ec-step1-theta}, \eqref{eq:ec-step1-node} and \eqref{eq:ec-step1-link}.} \nonumber
\end{IEEEeqnarray}

\begin{comment}
It is well-known that the McNaughton's algorithm~\cite{McNaughton59} solves the following scheduling problem optimally: given $n$ alike processors and $m$ independent tasks which take $a_1, \dots , a_m$ time to schedule on any one of the processors. The tasks can be preempted arbitrarily, but two processors cannot work on the same task as the same time.  The McNaughton's algorithm gives a schedule of minimum makespan equal to $\max\{\max\{a_i | 1 \le i \le m\}, \sum_{i = 1}^m a_i /m\}$. Suppose that an arc $e \in E(D)$ has the link time $t_e$, Then the minimum schedule time for a vertex $v \in V(D)$ is equal to 
\begin{equation}
t_v^* = \max\{ \max\{t_e / r(e) | e \in \delta_D(v)\}, \sum_{e \in \delta_D(v)} t_e / r(v) \},
\end{equation}
where $\delta_D(v)$ is the set of arcs in $D$ that are incident to $v$. A schedule of $t_v^*$ can be constructed by first dividing the task of scheduling each link $e \in \delta_D(v)$ into $r(e)$ tasks, each of time $t_e/r(e)$, and then applying the McNaughton's algorithm. 
Moreover, the schedule time for node $v$ cannot be less than $t_v^*$ because a link $e \in \delta_D(v)$ can have at most $r(e)$ pair of RF chains active, the schedule time for $e$ must be greater than or equal to $t_e / r(e)$ and the schedule time for $v$ must be greater than or equal to $\sum_{e \in \delta_D(v)} t_e / r(v)$ as $v$ has $r(v)$ number of RF chains. This proves that $t_v^*$ is the minimum schedule time for $v$.
\end{comment}

\subsection{Step (ii): Edge-coloring based Scheduling}
After we have obtained the link time, the next step is to generate a unit time schedule. Our  algorithm is based on the idea of multigraph edge coloring (a multigraph allows multiple edges between a pair of vertices). A proper edge coloring scheme assigns a color to each edge such that any two incident edges (sharing one or two vertices) are assigned different colors. Obviously, the set of edges $E_{\lambda}$ of a color $\lambda$ must be a matching in the multigraph. Hence $E_{\lambda}$  corresponds to a slot and an edge coloring scheme corresponds to a schedule. The EC algorithm takes a parameter {\em granularity} $t^g \in (0, 1]$, which is the quantization of the link time. A smaller $t^g$ typically leads to better schedule performance at the cost of longer execution time. Alg.~\ref{alg:ec-sched} lists the EC-based scheduling.
\begin{algorithm}[htbp]
	\textbf{Reduce graph}. Given the link time vector $\vect{t} = \{t_e | e \in E(D)\}$, we remove arcs in $D$ with zero link time and let the remaining graph be $D_r$\;
	\textbf{Split node}. We perform the node splitting in \S \ref{ss:node-split} on $D_r$. 
	Let the resulting graph be $D_s$. For each arc $e = (u, v) \in E(D_r)$ with link time $t_e$, we assign the link time
	$t_e / (r(u) \cdot r(v))$ to each arc $(u^{(i)}, v^{(j)})$ in $D_s$ for all combinations of $i = 1, \dots , r(u)$ 
	and $j = 1, \dots, r(v)$\; 	
	\textbf{Create multigraph and assign link time}. We create the
	coloring graph $D_m$, which has the same
	vertex set as $D_s$, and its arc set is defined as follows. For each $e = (u, v) \in E(D_s)$ with link time $t_e$, we install $\bigl\lceil t_e / t^g \bigr\rceil$ number of arcs $(u, v)$ in $D_m$. 
	$\bigl\lceil {t_e} / {t^g} \bigr\rceil-1$ of these arcs are
	assigned $t^g$ link time, and the last arc is
	assigned the remaining link time $t_e - (\bigl\lceil {t_e} / {t^g} \bigr\rceil-1) t^g$\;
	
	\textbf{Coloring and scheduling}. We perform edge coloring on
	$D_m$ (viewing $D_m$ as undirected). Suppose that $D_m$ can be colored with $\kappa$
	colors. For those arcs assigned the $i$-th color,
	$i=1,\ldots,\kappa$, we schedule the corresponding arcs in the $i$-th slot (each slot has the length $t^g$);
	
	\textbf{Scale}. The schedule is of length $\kappa t^g$. We scale the schedule by a factor of
	$1 / (\kappa t^g)$\;
	
	\caption{EC-based scheduling.}
	\label{alg:ec-sched}
\end{algorithm}

\subsection{Performance Analysis of the EC-based Scheduling}

The following lemma shows that step (ii) of the EC algorithm reduces the performance metric $\mu$ (in our case, max-min throughput $\theta$)  and link time $t_e$ of step (i) by a factor of ${1} / (\kappa t^g)$. Therefore, a better edge-coloring heuristic (smaller $\kappa$)~\cite{Nakano95} offers a better scheduling performance. 

\begin{lem} Suppose that before executing Line 3 of Alg.~\ref{alg:ec-sched},
	each link $e$ of $D_s$ has the link time $t_e$, and the performance metric
	is $\mu \ge 0$. Moreover, assume that if a schedule is scaled by $\gamma > 0$, then $\mu$ is also scaled by $\gamma$. 
	Then, after executing Alg.~\ref{alg:ec-sched}, the final link time is $t_e' = {t_e} / (\kappa t^g)$ and the final performance metric is $\mu' = {\mu} / (\kappa t^g)$.
	\label{lem:ec-quality}
\end{lem}
\begin{proof}
	Before scaling, the schedule is of length $\kappa t^g$.
	 To convert the schedule into unit length, we perform the scaling. Afterwards, $t_e' = {t_e} / (\kappa t^g)$ and $\mu' = {\mu} / (\kappa t^g)$.
\end{proof}

Since minimum edge coloring of an arbitrary graph is NP-complete~\cite{Holyer81}, we have to employ approximation algorithms. We choose the simple multigraph edge coloring algorithm by Karloff et al~\cite{Karloff87}. It uses at most $3\left \lceil \Delta(G)/2 \right \rceil$ colors, where $\Delta(G)$ is the maximal node degree of a multigraph $G$. The following lemma gives the upper bounds on $\Delta(D_m)$, the number of vertices $\card{V(D_m)}$ and arcs $\card{E(D_m)}$.
\begin{lem}
	$\Delta(D_m) < {1} / {t^g} +  r(D)$, 
	$\card{V(D_m)} \le r(D)$ and $\card{E(D_m)} < \frac{r(D)} {2 t^g} + \frac{ r(D)^2}{2}$.
	\label{lem:ec-bounds}
\end{lem}
\begin{proof}
	See Appendix~\ref{sec:lem:ec-bounds} for the proof.
\end{proof}

In the following, we will show the quality and time complexity of step (ii) of the EC algorithm. In practice, step (i) is much faster than step (ii).
\begin{thm}
	Let the performance metric after step (i) be $\mu \ge 0$. 
	In addition, assume that if a schedule is scaled by $\gamma > 0$, then $\mu$ is also scaled by $\gamma$.
	Then step (ii) achieves the performance metric $\mu' > \frac{2}{3 (r(D) + 2) t^g + 3 } \mu$ and it has time complexity of $O \bigl( ({r(D)} / {t^g}+r(D)^2) \log (r(D)+ {1} / {t^g})\bigr)$.
	\label{thm:ec-perf}
\end{thm}
\begin{proof}
	See Appendix~\ref{sec:thm:ec-perf} for the proof.
\end{proof}


Let the optimal max-min throughput of the FD-MTFS problem be $\theta^*$ (obtained by Alg.~\ref{alg:mtf-theta}). Since step (i) of the EC algorithm uses a looser constraint set than the one needed for computing  $\theta^*$, it gives a solution $\theta \ge \theta^*$. From Theorem~\ref{thm:ec-perf}, we have that the final max-min throughput of the EC algorithm $\theta' > \frac{2}{3(r(D) + 2)t^g + 3} \theta^*$.
In a typical backhaul network, we have $r(D) \gg 2$, so $\frac{2}{3(r(D) + 2)t^g + 3} \approx \frac{2}{3 r(D) t^g + 3}$. This means to keep a constant performance quality, we can choose $t^g = c / r(D)$ where $c$ is a constant. If $t^g$ is so selected, then the time complexity is $O(r(D)^2 \log r(D))$, which is quite scalable with $r(D)$ (total number of RF chains in $D$), and is hence feasible at a central controller.
Moreover, by setting $t^g$ close to 0, the final max-min throughput of the EC algorithm $\theta' > \frac{2}{3} \theta^*$.


==> fd-preliminary.tex <==
\section{Preliminary for full-duplex scheduling: schedule polytope}
\label{s:preliminary}
This section deals with the mathematical preliminary for the optimal polynomial time scheduling algorithm for full-duplex backhaul networks.
We first show the relation between a feasible schedule and matchings in a graph. Based on this relation, we mathematically formulate the set of all feasible schedules as the {\em schedule polytope} that is described by linear constraints.

\subsection{Node splitting} \label{ss:node-split}

The goal of {\em node splitting} is to prepare the directed network $D$ which has multi-RF-chain vertices, for scheduling. After performing node splitting on $D$, we obtain the {\em expanded network} $H$, a strict digraph on which scheduling can be performed directly. 
The node splitting is based on the idea that a node with $n$ RF chains is equivalent to $n$ nodes with a single RF chain each, among which data can be exchanged in zero time. 

$H$ is created by splitting each vertex $v \in V(D)$ into $r(v)$ vertices $v^{(1)},...,v^{(r(v))}$.
They are collectively called a {\em split vertex set} in $H$, which is denoted by $U(v) = \{v^{(i)} | i = 1,...,r(v)\}$. 
A split vertex set represents a BS. Let $B(H) = \cup_{v \in B(D)} U(v)$
and $M(H) = \cup_{v \in M(D)} U(v)$ be the set of all vertices in $H$ that belong to macro BSs and relay BSs respectively.
Moreover, each arc $e = (v, w) \in E(D)$ with capacity $c(e)$, is mapped to $r(v) \cdot r(w)$ number of arcs $\{ (v^{(i)}, w^{(j)}) | i = 1,...,r(v) \text{ and } j = 1,...,r(w)\}$ in $H$, each of which is assigned the same capacity $c(e)$. 
The function $u: V(H) \mapsto V(D)$ maps a split vertex in $H$ to a vertex in $D$ such that $u(v^{(i)}) = v$.
An example is shown in Fig.~\ref{fig:node-split}.
\begin{figure}[!t]
\centering
	\includegraphics[width=6cm]{figs/node-split.eps}
\caption{Node splitting. $u$ has 2 RF chains and $v$ has 3 RF chains. The vertices in a box are collectively called a {\em split vertex set}.}
\label{fig:node-split}	
\end{figure}

We observe that each feasible schedule $ S $ can be divided into  $ N \in \mathbb{N}$ timeslots numbered from 1 to $N$. Let $ t_i \in \mathbb{Q}_+$ denote the length of the $i$-th timeslot. It is required that $ \sum _ { i = 1 } ^ N t_i = 1 $.  Let a set of links (arcs) $E_i  \subseteq E(H)$ 
%($E_i$ can be empty) 
be scheduled in the $i$-th timeslot.
For full-duplex communication, the constraint that each node $v \in V(D)$ can serve at most $r(v)$ links (arcs) simultaneously is equivalent to the constraint that each node of $H$ can serve at most one link at a time. Thus, each $E_i$ is exactly a matching in $H$~\footnote{When we talk about a matching in $H$, we implicitly treat $H$ as an undirected graph by ignoring the arc orientations.}.

\begin{comment}
********************************

where $\delta(v)$ is the set of arcs incident to (entering or leaving) $v$ in $D$. As a result, the set of arcs of each timeslot $E_i$ is a b-matching in the graph $D$ where $b: V(D) \mapsto \mathbb{N}$ and $b(v) = r(v), \forall v \in V(D)$~\cite{Korte12}. 
{\em b-matching} of an undirected graph $G$ is defined as a set of edges $E \subseteq E(G)$ where $E$ is incident to each vertex $v \in V(G)$ for at most $b(v)$ times.

Let $\vect{x} \in \{0, 1\}^{E(H)}$ be the {\em incidence vector} of $E_i$, where an element $x_e = 1$ if $e \in E_i$ and $x_e = 0$ otherwise. 

********************************
\end{comment}

\subsection{The schedule polytope}
Let $\vect{t} \in \mathbb{R}_+^{E(H)}$ be a {\em link time vector} where $\mathbb{R}_+$ is the set of non-negative real numbers. Each element of $\vect{t}$ is the {\em link time} $t_e \in [0, 1]$ of an arc $e \in E(H)$, corresponding to the total active time of $e$.
A link time vector $\vect{t}$ is {\em feasible} if $\vect{t}$ can be scheduled in unit time. 
Next, we define the {\em schedule polytope} $P$ and then prove that each point in $P$ is one-to-one mapped to each feasible link time vector.


\begin{mydef}[Schedule Polytope] Given an expanded network $H$, the {\em schedule polytope} $P$ of $H$ is defined as the set of all link time vectors $\vect{t}$ that satisfy the  following linear constraints:
\begin{IEEEeqnarray}{rCll}
    \IEEEyesnumber\label{eq:link-active-time}\IEEEyessubnumber*
    \sum_{e \in \delta_H(v)}t_e & \le &1 &\qquad \forall\, v \in V(H),
    \label{eq:node-matching}\\
    \sum_{e \in E(H[O])} t_e & \le &
    \left \lfloor \frac{\card{O}}{2} \right\rfloor &\qquad
    \forall\, \text{odd set } O \subseteq   V(H), \label{eq:oddset} \\
    \vect{t}& \in &\mathbb{R}_+^{E(H)},
  \end{IEEEeqnarray}
where $\delta_H(v)$ is the set of arcs in $H$ that are incident to the vertex $v$. $H[O]$ is an {\em induced subgraph} of $H$ whose vertex set is $V(H[O]) = O$ and whose arc set $E(H[O])$ consists of all arcs in $H$ which have both ends in $O$. $O$ is an {\em odd set} if $|O|$ is an odd number.
\end{mydef}


The following lemma summarizes the relation between the schedule polytope and a feasible unit length schedule.

\begin{lem} Given an expanded network $H$, (i) each point in the schedule polytope $P$ is a feasible link time vector $\vect{t}$, and (ii) each feasible link time vector $\vect{t}$ is a point in $P$.
\label{lm:schedule-matching}
\end{lem}
\begin{proof}
%The proof uses the Edmonds' matching polyhedron theorem~\cite{Edmonds65b}. A feasible schedule $S$ consists of $N \in \mathbb{N}$ timeslots. Each timeslot contains a set of arcs from $H$ that is a matching and therefore corresponds to a vertex of the matching polytope $Q$. Since $Q$ has the same formulation as $P$, $P$ and $Q$ share the same set of vertices. Since $S$ has unit length, the link time vector $\vect{t}$ of $S$ is a convex combination of the vertices of $P$ and thus is a point in $P$. On the other hand, a point in $P$ can be written as a convex combination of all vertices of $P$ where each vertex corresponds to the set of arcs scheduled in a timeslot. Therefore, each point in $P$ corresponds to a feasible unit time schedule. The number of timeslots in the schedule is at most the number of vertices of $P$.
 See Appendix~\ref{sec:proof_lemma1} for the proof.  
\end{proof}

\begin{comment}
\subsection{Special case of no links between mmBSs} 
If the system model allows no links between mmBSs, then $G$ is a bipartite graph (the set of expanded eNBs $\set{R}$ and the set of mmBSs $\set{W}$ are the two parts). For bipartite graphs, the odd set constraints \eqref{eq:oddset} are redundant for the schedule polyhedron since they are redundant for the matching polytope~\cite{Birkhoff46}. 
By removing the constraints \eqref{eq:oddset}, whose number is exponential to $|\set{V}|$, from \eqref{eq:link-active-time}, we can improve the runtime efficiency of the optimization algorithms.  
After the removal, Lemma~\ref{lm:schedule-matching} is still valid.

\end{comment}


==> hd-approx-algo.tex <==
\section{Approximation Algorithms for Half-Duplex Maximum Throughput Fair Scheduling}
\label{s:hd-approx-algos}


 the HD-MTFS problem is NP-complete in general (see \S \ref{s:hd-mtfs}), we have to rely on polynomial-time approximation algorithms
for the solution.



\subsection{Approximation Algorithms based on Fractional Weighted Coloring}
The two approximation algorithms in this subsection are based on the method of {\em fractional weighted vertex coloring} of {\em conflict graphs} as proposed by Wan et al~\cite{Wan09}.

A half-duplex backhaul scheduling problem can be transformed to a fractional weighted vertex coloring problem since both the half-duplex constraint and the RF chain number constraint can be modeled by the conflict graph.

Given a directed network $D$, we create the {\em sparsely expanded network} $H^s$ in the same way as the {\em expanded network} $H$ with one exception: if an arc $e = (u,v) \in E(D)$ has the same number of RF chains at both ends, i.e., $r(u) = r(v)$, $e$ is mapped to exactly $r(u)$ arcs in $H^s$, $\{(u^{(i)}, v^{(i)}) | \forall i\}$. An example in shown in Fig.~\ref{fig:sparse-ex-net}. Compared with an expanded network, a sparsely expanded network has less arcs which can significantly reduce runtime of optimization algorithms. However, we first need to prove that the sparsely expanded network can substitute the expanded network for scheduling.

\begin{figure}[hbpt]
	\centering
	\includegraphics[width=8.8cm]{figs/sparse-expanded-network.eps}
	\caption{Transform a directed network $D$ into a sparsely expanded network $H^s$. The number inside a node is its number of RF chains.}
	\label{fig:sparse-ex-net}	
\end{figure}

\begin{thm}
	Given a directed network $D$, suppose its multi-arc network is $F$ and its sparsely expanded network is $H^s$. Then any half-duplex subgraph of $F$ can be represented by a matching in $H^s$.
	\label{thm:sparse-exp-net}
\end{thm}
\begin{proof}
	See Appendix~\ref{sec:thm:sparse-exp-net} for the proof.
\end{proof}

Assume that each arc $e \in E(H^s)$ needs to be scheduled for a link time $t_e \in \mathbb{R_+}$. How to compute the link time vector $\vect{t} = [t_e|e \in E(H^s)]$ will be discussed later.
The conflict graph $C$ is constructed as follows: initially, $C$ is equal to the line graph\footnote{Given a graph $G$, its line graph $L(G)$ is a graph such that (i) each vertex of $L(G)$ represents an edge of $G$, and (ii) two vertices of $L(G)$ are adjacent if and only if their corresponding edges are incident in $G$.} of $H^s$ (viewing $H^s$ as undirected), which models the RF chain number constraint. Then, we add additional edges to $C$, to model the half-duplex constraint. Specifically, for each pair of non-incident arcs $(p, q), (s, t) \in E(H^s)$ such that $u(q) = u(s)$ or $u(t) = u(p)$, we add an undirected edge between two vertices $(p, q)$ and $(s, t)$ in $C$. Adjacent vertices in $C$ cannot be scheduled simultaneously because they are in {\em conflict}. The conflict graph for the sparsely expanded network in Fig.~\ref{fig:sparse-ex-net} is shown in Fig.~\ref{fig:conflict-graph}.
\begin{figure}[hbpt]
	\centering
	\includegraphics[width=5cm]{figs/conflict-graph.eps}
	\caption{Conflict graph $C$ of the sparsely expanded network $H^s$ in Fig.~\ref{fig:sparse-ex-net}. The solid and dashed edges represent the RF chain number constraints and the half-duplex constraints, respectively. }
	\label{fig:conflict-graph}	
\end{figure}


The {\em minimum makespan} scheduling for a link time vector $\vect{t} = [t_e | e \in E(H)] = [t_v | v \in V(C)]$ is the same as the {\em minimum fractional weighted coloring} of $(C, \vect{t})$. The latter is defined as a set of $K \in \mathbb{N}$ pairs $(I_i, \lambda_i)$ where each $I_i$ is an independent set (a set of nonadjacent vertices) of $C$  and $\lambda_i \in \mathbb{R}_+$ for $1 \le i \le K$ satisfying that $\sum_{1 \le i \le K, v \in I_i} \lambda_i = t_v, \forall v \in V(C)$ and the sum $\sum_{i = 1}^K \lambda_i$ is at the minimum. But the problem of finding minimum fractional weighted coloring is NP-complete~\cite{Groetschel81}. Let $P$ be the {\em independence polytope} of $C$, i.e., the convex hull of the incidence vectors
 of the independent sets of $C$. Any point in $P$ corresponds to a feasible unit time schedule. The minimum fractional weighted coloring problem can be expressed as a linear program with the help of $P$.
 The {\em fractional chromatic number} $\chi_f(C, \vect{t})$ is defined as the minimum weight of the coloring, $\sum_{i=1}^K \lambda_i$.

We use the results of~\cite{Wan09} and propose two approximation algorithms based on fractional weighted coloring. 
The difference of the two algorithms lies in the linear programs for computing the link time vector $\vect{t}$ and the ordering of the vertices $V(C)$ for coloring. The coloring step uses the so-called {\em first-fit fractional weighted coloring} (F$^3$WC) algorithm from~\cite{Wan09}, listed in Alg.~\ref{alg:f3wc}.

\begin{algorithm}[!t]
	\SetAlgoLined
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	
	\Input{$C$, $\vect{t} \in \mathbb{R}_+^{V(C)}$, and an ordering of $V(C)$.}
	\Output{A fractional weighted coloring $\Pi$ of $(C, \vect{t})$.}
	
	$\Pi \leftarrow \emptyset$\;
	$U \leftarrow \{v \in V(C) | t_v > 0\}$\;
	
	\While{$U \ne \emptyset$} {
		$I \leftarrow$ the first-fit MIS (maximal independent set) of $U$\;
		$\lambda \leftarrow \min_{v \in I} t_v$\;
		add $(I, \lambda)$ to $\Pi$\;
		\For{each $v \in I$} {
			$t_v \leftarrow t_v - \lambda$\;
			\If{$t_v = 0$}
			{remove $v$ from $U$\;}
		} 
	}
	output $\Pi$\;
	\caption{First-fit fractional weighted coloring.}
	\label{alg:f3wc}
\end{algorithm}

\subsubsection{Fixed and arbitrary ordering (F$^3$WC-FAO)} \label{sec:hd-f3wc-fao}
Assume that $\langle v_1, \dots , v_n \rangle$ is an arbitrary but fixed ordering of $V(C)$ where $n = \card{V(C)}$.
We denote $v_i < v_j$ if $i < j$.
Let $V_i$ be the set of vertices of $v_i$ and all its neighbors in $\{v_1, \dots , v_{i-1}\}$.
Define the {\em inductive independence polytope} $Q$ of $C$ by the ordering $\langle v_1, \dots, v_n \rangle$ as
\begin{equation}
	Q \eqdef \Big \{ \vect{t} \in \mathbb{R}_+^{V(C)} \Big| \max_{1 \le i \le n} t(V_i) \le 1 \Big \},
\end{equation}
where $t(V_i) = \sum_{v \in V_i} t_v$. We say $Q$ is an approximation of the independence polytope $P$.

\begin{lem}
	Let $D$ be a directed network. We have $Q \subseteq P \subseteq \alpha^*Q$ where $\alpha^* \le \max_{(u, v) \in E(D)} [ r(u) + r(v) ]$.
	For any $\vect{t} \in Q$, the coloring of $(C, \vect{t})$ by F$^3$WC-FAO has weight at most 1.
	\label{lem:Q}
\end{lem}
\begin{proof}
	See Appendix~\ref{sec:lem:Q} for the proof.
\end{proof}


\subsubsection{Largest surplus last ordering (F$^3$WC-LSLO)} \label{sec:hd-f3wc-lslo}
The largest surplus last ordering of $V(C)$ is done by first transforming the undirected graph $C$ into a directed graph 
$C^d$ by imposing the following orientation on each edge $e \in E(C)$.

Suppose that the vertices of the directed network $D$ has an ordering. That is, given two different vertices $w, w' \in V(D)$, if $w$ comes before $w'$ in the ordering, we have $w < w'$. 
We specify that given two different vertices $u^{(i)}$ and $v^{(j)}$ of the sparsely expanded network $H^s$, 
we have $u^{(i)} < v^{(j)}$ if and only if $u < v$ or ($u = v$ and $i < j$).
 In addition, given two different vertices $(u^{(i)}, v^{(j)})$ and $(s^{(k)}, t^{(l)}) \in V(C^d)$, $(u^{(i)}, v^{(j)}) < (s^{(k)}, t^{(l)})$, if and only if $u^{(i)} < s^{(k)}$ or 
$(u^{(i)} = s^{(k)}$ and $v^{(j)} <  t^{(l)})$.

The orientation is chosen according to the following rules for each edge in $C$:
\begin{enumerate}
	%\item An edge between $(u^{(i)}, v^{(j)})$ and a vertex of the form $(x^{(k)}, u^{(l)})$ such that $v \ne x$ has the orientation from $(x^{(k)}, u^{(l)})$ to $(u^{(i)}, v^{(j)})$.
	\item An edge between $(u^{(i)}, v^{(j)})$ and a vertex of the form $(v^{(k)}, x^{(l)})$ such that $u \ne x$ has the orientation
	from $(u^{(i)}, v^{(j)})$ to $(v^{(k)}, x^{(l)})$.
	\item An edge between $(u^{(i)}, v^{(j)})$ and a vertex of the form $(u^{(i)}, x^{(l)})$ or $(x^{(k)}, v^{(j)})$ or $(v^{(k)}, u^{(l)})$ has the orientation from the smaller vertex to the bigger vertex.
\end{enumerate}

Let $D'$ be a digraph. 
For each $u \in V(D')$, let $N^{in}(u)$ denote the set of in-neighbors of $u$ in $D'$, and let $N^{in}[u]$ denote $\{u\} \cup N^{in}(u)$.
For any $\vect{t} \in \mathbb{R}_+^{V(D')}$, the {\em surplus} of a vertex $u$ is defined as $t(N^{in}(u)) - t(N^{out}(u))$.
The largest surplus last ordering is constructed as follows. Let $\vect{t} \in \mathbb{R}_+^{V(C^d)}$. Initialize $D'$ to $C^d$. For $i = n$ down to 1, let $v_i$ be a vertex of the largest surplus in $(D', \vect{t})$ and then delete $v_i$ from $D'$ and the element $t_{v_i}$ from $\vect{t}$.
The ordering of $\langle v_1, \dots , v_n \rangle$ is the largest surplus last ordering of $(C^d, \vect{t})$.
The {\em independence polytope} $Q'$ of $C^d$ is defined as 
\begin{equation}
	Q' = \Big \{ \vect{t} \in \mathbb{R}_+^{V(C^d)} \Big | \max_{u \in V(C^d)} t (N^{in}[u]) \le 1/2 \Big \},
\end{equation}
which is an approximation of the independence polytope $P$.

\begin{lem}
	Let $D$ be the directed network and $r_{max} = \max_{u \in V(D)} r(u)$ be the maximum RF chain number of any BS in $D$, we have $Q' \subseteq P \subseteq 2 \beta^* Q'$ where $\beta^* \le r_{max} + 1$.
	For any $\vect{t} \in Q'$, the coloring of $(C, \vect{t})$ by F$^3$WC-LSLO has weight at most 1.
	\label{lem:Q'}
\end{lem}
\begin{proof}
	See Appendix~\ref{sec:lem:Q'} for the proof.
\end{proof}

A fractional weighted coloring based approximation algorithm consists of three steps: (i) computing the link time vector 
$\vect{t} = [t_e | e \in E(H^s)]$, (ii) sorting the vertices $V(C)$ and performing F$^3$WC on the given ordering, and (iii) scaling the schedule.

We assume that there is a sorting method which has a corresponding $\gamma$-approximate ($\gamma > 1$) independent polytope $Q^\circ$, 
i.e., $Q^\circ \subseteq P \subseteq \gamma Q^\circ$. 
Specifically, we have two options---fixed and arbitrary ordering or largest surplus last ordering with $\gamma = \alpha^*, Q^\circ = Q$ 
and $\gamma = 2\beta^*, Q^\circ = Q'$, respectively. Step (i) is to solve the following two linear programs.
\begin{IEEEeqnarray}{lrClr}
	\label{eq:q0app1}
	\IEEEyesnumber \IEEEyessubnumber* 
	\textnormal{max} & \theta & & & \\
	\textnormal{s.t.} &\sum_{\mathclap{e\in\delta_{H^s}^-(U(v))}} c(e) t_e
	-\sum_{\mathclap{e\in\delta_{H^s}^+(U(v))}} c(e) t_e& \ge & \theta
	\quad\forall\,v\in M(D)\IEEEeqnarraynumspace \label{eq:q0app-maxmin-tput}
	\\
	& \vect{t} & \in & Q^\circ \IEEEeqnarraynumspace \label{eq:q0app-in-q0}
\end{IEEEeqnarray}

With the max-min throughput solution $\theta$, we go on to compute $\vect{t}$ for the maximum network throughput.
\begin{IEEEeqnarray}{lC}
	\IEEEyesnumber \IEEEyessubnumber*
  	\textnormal{max} &\sum_{\mathclap{e \in \{\delta_{H^s}^+(U(v)) | v \in B(D) \}}} c(e) t_e
\nonumber\\
	\textnormal{s.t.}& \eqref{eq:q0app-maxmin-tput} \text{ and } \eqref{eq:q0app-in-q0}. \nonumber \IEEEeqnarraynumspace 
\end{IEEEeqnarray}
Step (ii) is to sort $V(C)$ with the given method and then to perform the F$^3$WC algorithm (Alg.~\ref{alg:f3wc}) 
with the computed $\vect{t}$ and vertex ordering. 
Since, it is guaranteed by step (i) and (ii) that the schedule length after performing the F$^3$WC algorithm is no more than one, we perform the last step to scale the schedule length to exactly unit time. The goal is to  improve performance by fully utilizing the available time resource.
Next, we will show the worst-case max-min throughput achieved by the approximation algorithms.

\begin{thm}
	The algorithms F$^3$WC-FAO and F$^3$WC-LSLO solve the HD-MTFS problem by producing a unit-time schedule.
	They achieve a max-min throughput $\theta' \ge \theta^*/\alpha^*$ and $\theta' \ge \theta^* / (2 \beta^*)$ respectively,
	where $\theta^*$ is the optimum. 
	\label{thm:perf-f3wc}
\end{thm}
\begin{proof}
	See Appendix~\ref{sec:thm:perf-f3wc} for the proof.
\end{proof}


In summary, the three algorithms---a) PLS, 
b) F$^3$WC-FAO and c) F$^3$WC-LSLO are respectively $\frac{r_{min}}{\max\{r_{max}^M, \max_{v \in B(D)} m(v)\}}$,
$1/\max_{(u,v) \in E(D)} [r(u) + r(v)]$ and $1/(2r_{max}+2)$-approximate algorithms for the HD-MTFS problem, where a $\rho$-approximate ($\rho \le 1$) algorithm achieves a max-min throughput $\theta$ that is at least $\rho$ times of the optimal value $\theta^*$, 
$\theta \ge \rho \theta^*$.
Theoretically, PLS has the best performance and F$^3$WC-LSLO has the worst.



==> hd-sched-fair.tex <==
\section{Half-duplex maximum throughput fair scheduling}
\label{s:hd-mtfs}
In this section, we will study the {\em half-duplex maximum throughput fair scheduling} (HD-MTFS)  problem. 
Different from the polynomial-time solvable problem FD-MTFS, HD-MTFS is NP-complete, which will be proved in \S \ref{ss:hd-mtfs-np-comp}.
 Then we will study the special case that all relay BSs have the same number of RF chains $r^M$ and any macro BS has the RF chain number that is a multiple of $r^M$. The special case allows polynomial-time optimal solution.

\subsection{Linear Programs for HD-MTFS Problem}
Compared to the FD-MTFS problem, the HD-MTFS problem has the additional {\em half-duplex} constraint---a BS cannot work as transmitter and receiver at the same time. Due to this constraint, the matching-based optimization method that works successfully for the full-duplex case cannot be applied.

To prepare for the analysis, we first transform a {\em directed network} $D$ into a {\em multi-arc network} $F$ as follows. $F$ has the same vertex set as $D$, $V(F) = V(D)$. Each arc $e = (u, v) \in E(D)$ is mapped into $\min\{r(u), r(v)\}$ number of parallel arcs $(u, v)$ in $F$, each of which has the same capacity as $c(e)$. As a consequence, $F$ is transformed from $D$ by simply duplicating the arcs in $D$. Let $B(F) = B(D)$ and $M(F) = M(D)$ be the set of macro BSs and the set of relay BSs, respectively. 

For full-duplex scheduling, the links scheduled in each timeslot forms a matching in the expanded network $H$. Correspondingly, for half-duplex scheduling, the links scheduled in each timeslot forms a subgraph $J \subseteq F$ subject to the following constraints. We call $J$ a {\em half-duplex subgraph} of $F$.
\begin{mydef}[Half-duplex Subgraph] A half-duplex subgraph of a multi-arc network $F$ is a subgraph $J \subseteq F$ such that (i) $J$ is a {\em directed bipartite graph}, i.e., $V(J)$ can be divided into two disjoint sets $V_1, V_2$ where each arc of $E(J)$ has the head in $V_2$ and the tail in $V_1$ and (ii) $J$ satisfies the vertex degree constraint of $d_J(v) \le r(v), \forall v \in V(J)$, where $d_J(v)$ is the degree of $v$ in graph $J$.
\end{mydef}
The constraint \emph{(i)} reflects the half-duplex constraint, because the active nodes for a timeslot can be divided into the sender set $V_1$ and the receiver set $V_2$, where links only go from a sender to a receiver. The constraint \emph{(ii)} is due to the fixed number of RF chains.
Analogous to the node-matching matrix, we define the {\em node-hd-subgraph matrix} for the formulation of the HD-MTFS problem.
\begin{mydef} [Node-hd-subgraph Matrix] Given a multi-arc network $F$, suppose that the number of all half-duplex subgraphs of $F$ is $K$. Then the node-hd-subgraph matrix $\mat{L} = [l_{i, j}]$ is a $|V(F)| \times K$ matrix. Denote the $i$-th vertex of $F$ as $v_i$, which is related to the $i$-th row of $\mat{L}$. 
	Denote the $j$-th half-duplex subgraph of $F$ as $J_j$, which is related to the $j$-th column of $\mat{L}$.
	 Each element $l_{i, j}$ is equal to the sum capacity of all arcs in $J_j$ that enter $v_i$ minus the sum capacity of all arcs in $J_j$ that leave $v_i$.
\end{mydef}
\begin{figure}[!t]
\begin{minipage}{0.12\textwidth}
\begin{figure}[H]
	\includegraphics[width=2cm,left]{figs/node-hd-subgraph.eps}	
\end{figure}
\end{minipage} \hspace{-0.5cm}
$L:$
\begin{minipage}{0.3\textwidth} \footnotesize
$\begin{blockarray}{cccccccc}
         & \alpha  & \beta  & \gamma   & \delta  & \alpha, \beta & \alpha, \delta & \beta, \delta   \\
  \begin{block}{c[ccccccc]}
    v_0  & -8 & -8 & 0   & 0  & -16 & -8  & -8 \\
    v_1  & 8  & 8  & -3  & 3  & 16  & 11  &  11 \\
    v_2  & 0  & 0  & 3   & -3 & 0   & -3  &  -3 \\
  \end{block}
\end{blockarray}$
\end{minipage}
\caption{Node-hd-subgraph matrix $\mat{L}$. $v_0, v_1$ and $v_2$ have 2, 2 and 1 RF chain respectively. The arc capacities are: 
	$c(\alpha) = c(\beta) = 8$, $c(\gamma) = c(\delta) = 3$.}
\label{node-hd-subgraph}
\end{figure}
Fig.~\ref{node-hd-subgraph} gives an example of the node-hd-subgraph matrix for a multi-arc network. Similar to the definition of $\mat{A}^M$ in \S \ref{ss:sched-ori-opt}, $\mat{L}^M$ is the submatrix of $\mat{L}$ that only consists
of the rows of $\mat{L}$ related to relay BSs. 

The linear program formulation of the HD-MTFS problem is the same as \eqref{eq:mtf-theta} and \eqref{eq:mtf} except that $\mat{A}^M$ is replaced by $\mat{L}^M$ and $\vect{c}$ is adjusted accordingly:
\begin{IEEEeqnarray}{lrCl}
  \IEEEyesnumber\label{eq:hd-mtf-theta}\IEEEyessubnumber*
  \textnormal{max} & \theta & &
  \\
  \textnormal{s.t.}\quad& \mat{L}^{M}\vect{t}^S& \geq & \vect{1}\theta
  \\
  & \trans{\vect{1}}\vect{t}^S& = &1
  \textnormal{ and }
   \vect{t}^S \geq \vect{0},
\end{IEEEeqnarray}
\begin{IEEEeqnarray}{lrCl}
  \IEEEyesnumber\label{eq:hd-mtf}\IEEEyessubnumber*
  \textnormal{max} &\trans{\vect{c}}\vect{t}^S & &
  \\
  \textnormal{s.t.}\quad& \mat{L}^{M}\vect{t}^S& \geq & \vect{1} \theta^*
  \\
  & \trans{\vect{1}}\vect{t}^S& = &1
  \textnormal{ and }
   \vect{t}^S \geq \vect{0},
\end{IEEEeqnarray}
 
However, different from the polynomial-time solvable FD-MTFS problem, the HD-MTFS problem can be shown as NP-complete.

\subsection{HD-MTFS Problem is NP-complete} \label{ss:hd-mtfs-np-comp}
\begin{mydef} [Maximum Capacity Half-duplex Subgraph (MCHS) Problem] Given a multi-arc network $F$, find a half-duplex subgraph $J \subseteq F$ such that $\sum_{e \in E(J)} c(e)$ is maximized.
\end{mydef}
Since the maximum matching problem can be solved in polynomial time, so is the FD-MTFS problem (see \S \ref{s:fd-sched-fair}). Analogously, if the MCHS problem can be solved in polynomial time, so is the HD-MTFS problem (\eqref{eq:hd-mtf-theta} and \eqref{eq:hd-mtf}).
 Unfortunately, this is not the case. The MCHS problem is NP-complete for a multi-arc network even if it a directed acyclic graph (DAG). Furthermore, by extending the technique for proving NP-completeness of MCHS, we can prove that the HD-MTFS problem is also NP-complete.

\begin{lem} The MCHS problem is NP-complete on a directed acyclic multi-arc network.
\label{lem:MCHS-DAG}
\end{lem}
\begin{proof} The proof is done by reduction from the SAT problem. For more detail, see Appendix~\ref{sec:proof-lem-MCHS-DAG}.
\end{proof}

%Next, we show that the HD-MTFS problem is NP-complete,
\begin{thm}
The HD-MTFS problem is NP-complete for a general directed network.
\label{thm:HD-MTFS-NP-complete}	
\end{thm}
\begin{proof}
	See Appendix~\ref{sec:proof-thm-HD-MTFS} for the proof.
\end{proof}
In general, the optimal scheduling of mmWave backhaul network can be solved in polynomial time when all BSs are full-duplex.
In contrast, the problem is NP-complete when all BSs are half-duplex, i.e., it is impossible to obtain an optimal schedule in polynomial time.
%The FD-MTFS problem can be solved optimally in polynomial time, but the HD-MTFS problem is NP-complete, i.e., it is impossible to obtain an optimal solution in polynomial time. 
%Moreover, according to the proof of Theorem~\ref{thm:HD-MTFS-NP-complete}, HD-MTFS is NP-complete even if the directed network has the propoerty that between any pair of vertices there are either zero or two opposite arcs of the  same capacity.

\subsection{Special Case HD-MTFS is Solvable in Polynomial Time} \label{sec:hd-mtfs-special-case}
We now investigate the special case that HD-MTFS is solvable in polynomial time. 
It is so when the backhaul network has {\em uniform RF chains}. After we have proved it, we will extend the polynomial-time solvable condition.
\begin{mydef}[Uniform RF chains] Given a directed network $D$, if the RF chain number function $r(v) \equiv R \in \mathbb{N}$, $\forall v \in V(D)$, we say $D$ has {\em uniform RF chains}.
\end{mydef}

Obviously, HD-MTFS is solvable in polynomial time for the case of {\em single uniform RF chain}, i.e., $r(v) \equiv 1$, $\forall v \in V(D)$, because the half-duplex constraint is automatically satisfied if each node can serve at most one directed link.
Thus, the optimal schedule can be obtained with the OPT-FD-MTFS algorithm.
 Next we will prove that HD-MTFS is also solvable in polynomial time for the case of uniform RF chains.
\begin{lem} Assume that an undirected loopless multigraph $G$ has the property that between each pair of vertices $u, v \in V(G)$, there are either $R \in \mathbb{N}$ edges of the same positive weight $w(\{u, v\})$ or zero edges. The maximum weight biparite subgraph $J \subseteq G$ such that each vertex $v \in V(J)$ has degree $d_J(v) \le R$, can be found in polynomial time as follows:
\begin{enumerate}
	\item Create the related simple graph $G'$ for $G$: between each pair of vertices $u, v \in V(G)$, if there are $R$ edges, we only keep one of them. Let the resulting graph be $G'$.
	\item Find the maximum weight matching $M$ of $G'$ with the weight function $w$. The maximum weight bipartite subgraph $J$ is the graph whose edge set is the multiset $(M, R)$, i.e., $R$-time repetition of $M$.
\end{enumerate}
\label{lem:max-bipartite-subgraph}
\end{lem}
\begin{proof}
	See Appendix~\ref{sec:lem:max-bipartite-subgraph} for the proof.
\end{proof}

Based on the above lemma, we propose the algorithm for solving the HD-MTFS problem when the backhaul network has uniform RF chains in the following theorem.
\begin{thm}
	Given a directed network $D$ and a uniform RF chain function $r(v) \equiv R$, $\forall v \in V(D)$, the HD-MTFS problem can be solved in polynomial time as follows:
\begin{enumerate}
	\item Compute the optimal schedule $S$ with the OPT-FD-MTFS algorithm on the directed network $D$ assuming that each vertex has a single RF chain.
	\item The optimal schedule $S^*$ is $R$ copies of $S$ running in parallel.
\end{enumerate}
\label{thm:hd-mtfs-uniform-rf}
\end{thm}
\begin{proof}
	See Appendix~\ref{sec:thm:hd-mtfs-uniform-rf} for the proof.
\end{proof}

We can extend the condition of uniform RF chains to that each relay BS has the same number of RF chains $r^M$ and the number of RF chain of any macro BS is a multiple of $r^M$.

\begin{cor}
Given a directed network $D$, assume that each relay BS has the same number of RF chains, $r(v) \equiv r^M \in \mathbb{N}, \forall v \in M(D)$. In addition, we assume that any macro BS has RF chain number that is a multiple of $r^M$, i.e., for each $i = 1, \dots, \card{B(D)}$ and $n_i \in B(D)$, $r(n_i) = k_i \cdot r^M$, where $k_i \in \mathbb{N}$. The optimal solution to the HD-MTFS problem on $D$ can be solved in polynomial time as follows:
\begin{enumerate}
	\item Replace each macro BS vertex $n_i$ by $k_i$ vertices $n_i^{(1)}, \dots, n_i^{(k_i)}$,  each of which has $r^M$ RF chains. Each vertex $n_i^{(j)}$ is connected with the same set of nodes and with the same arc capacities as $n_i$. Let the resulting directed network be $D'$.
$D'$ satisfies the condition of uniform RF chains.
	\item The optimal HD-MTFS schedule on $D$ is equivalent to the optimal HD-MTFS  schedule on $D'$.
\end{enumerate}
\label{cor:uni-rf-sched}
\end{cor}
\begin{proof}
	The optimal schedule for $D$ is equivalent to the optimal one for $D'$, since a macro BS $n_i$ never acts as a receiver.
\end{proof}





==> intf-approx-algo.tex <==
\section{Approximation Algorithms for the Pairwise Link Interference Model}
Till now, we have assumed that there is no interference between concurrent links. 
In this section, we will discuss scheduling algorithms by taking into account the pairwise link interference model described in Sec.~\ref{s:sysmodel}.
We will first show that the MTFS problem is NP-complete and then we will show how to adapt the fractional weighted coloring based approximation algorithms to consider the interference.

\subsection{Adaptation of Fractional Weighted Coloring Based Approximation Algorithms}
Since both FD-MTFS and HD-MTFS problems are NP-complete under the given interference model, we need approximation algorithms for the scheduling.
Fortunately, the fractional weighted coloring based approximation algorithms F$^3$WC-FAO and F$^3$WC-LSLO are readily adaptable to the pairwise link interference model.

\subsubsection{FD-MTFS}
Given a directed network $D$, we create the {\em expanded network} $H$. We cannot use the {\em sparsely expanded network} $H^s$ because it only applies to the half-duplex scheduling (see Theorem~\ref{thm:sparse-exp-net}).

The modification to the algorithm F$^3$WC-FAO in Sec~\ref{sec:hd-f3wc-fao} is only in the construction of the conflict graph $C$.
We construct $C$ that is the line graph of $H$, which models the RF chain number constraint. 
For each pair of interfering links $e_1$ and $e_2$ in $D$, suppose they are expanded to the arc sets $E_1$ and $E_2$ in $H$ respectively.
Then we add $|E_1| \cdot |E_2|$ edges to $C$. Each edge is between two vertices in $C$ that represent one arc in $E_1$ and one arc in $E_2$.

The modification to the algorithm F$^3$WC-LSLO in Sec~\ref{sec:hd-f3wc-lslo} is only in the orientation rules of the directed conflict graph $C^d$.
$C^d$ is transformed from the undirected conflict graph $C$ in the last paragraph according to the following orientation rules for each edge in $C$:
\begin{enumerate}
	%\item An edge between $(u^{(i)}, v^{(j)})$ and a vertex of the form $(x^{(k)}, u^{(i)})$ such that $v \ne x$ has the orientation from $(x^{(k)}, u^{(i)})$ to $(u^{(i)}, v^{(j)})$.
	\item An edge between $(u^{(i)}, v^{(j)})$ and a vertex of the form $(v^{(j)}, x^{(l)})$ such that $u \ne x$ has the orientation
	from $(u^{(i)}, v^{(j)})$ to $(v^{(j)}, x^{(l)})$.
	\item An edge between $(u^{(i)}, v^{(j)})$ and a vertex of the form $(u^{(i)}, x^{(l)})$ or $(x^{(k)}, v^{(j)})$ or $(w^{(k)}, y^{(l)})$ such that $u \ne v \ne w \ne y$ has the orientation from the smaller vertex to the bigger vertex.
\end{enumerate}

\subsubsection{HD-MTFS}
Given a directed network $D$, we create the {\em sparsely expanded network} $H^s$. 

The modification to the algorithm F$^3$WC-FAO in Sec~\ref{sec:hd-f3wc-fao} is to add one last step to the construction of the conflict graph $C$.
That is for each pair of interfering links $e_1$ and $e_2$ in $D$, suppose they are expanded to the arc sets $E_1$ and $E_2$ in $H^s$ respectively.
Then we add $|E_1| \cdot |E_2|$ edges to $C$. Each edge is between two vertices in $C$ that represent one arc in $E_1$ and one arc in $E_2$.

The modification to the algorithm F$^3$WC-LSLO in Sec~\ref{sec:hd-f3wc-lslo} is to change the second orientation rule as the following (the first rule is kept unchanged):
\begin{enumerate}
	\setcounter{enumi}{1}
	\item An edge between $(u^{(i)}, v^{(j)})$ and a vertex of the form $(u^{(i)}, x^{(l)})$ or $(x^{(k)}, v^{(j)})$ or $(v^{(k)}, u^{(l)})$
	or $(w^{(k)}, y^{(l)})$ such as $u \ne v \ne w \ne y$ has the orientation from the smaller vertex to the bigger vertex.
\end{enumerate}

\subsubsection{Approximation Results Considering Link Interference}
Obviously, the worst-case performance of the fractional weighted coloring based approximation algorithms depends on the state of pairwise link interference. Therefore, the results in Theorem~\ref{thm:perf-f3wc} does not apply since it assume no interference.
Yet the general lower bounds from~\cite{Wan09} still hold.
We define the {\em inductive independence number} of a conflict graph $C$ as the maximum size of any independent set of $C$ contained in some $V_i$. $V_i$ is
the set containing vertex $v_i$ and all its neighbors in $\{v_1 \dots v_{i-1}\}$ where $\langle v_1 \dots  v_n \rangle$ is a fixed ordering of $V(C)$.
We define the {\em local independence number} of a directed conflict graph $C^d$ as the maximum size of any independent set of $C^d$ contained in $N^{in}[u]$ for some $u \in V(C^d)$ where $N^{in}[u]$ is the set containing $u$ and its in-neighbors.
\begin{thm}
	Given the pairwise link interference model, the algorithms F$^3$WC-FAO and F$^3$WC-LSLO solve the MTFS problem by producing a unit-time schedule. They achieve a max-min throughput $\theta' \ge \theta^* / \alpha^*$ and $\theta' \ge \theta^*/(2\beta^*)$ respectively where $\theta^*$ is the optimum. 
	$\alpha^*$ is the {\em inductive independence number} of $C$ and $\beta^*$ is the {\em local independence number} of $C^d$.
\end{thm}
\begin{proof}
	The proof follows directly from~\cite{Wan09}.
\end{proof}

==> real-su-sm.tex <==
\section{Algorithms for the REAL-SU-SM Model}
This section deals with the MTFS scheduling algorithms (optimal and approximation) assuming the single user spatial multiplexing model MAX-SU-SM (see Sec.~\ref{sec:su-sm}).

\subsection{Optimal FD-MTFS Scheduling Algorithm Assuming NI Model and REAL-SU-SM Model}
This section is actually an extension of the optimal FD-MTFS scheduling algorithm in Sec.~\ref{s:fd-sched-fair}.
The difference in the problem setting is that in  Sec.~\ref{s:fd-sched-fair} we assume the MAX-SU-SM model while in this section we assume REAL-SU-SM model.
In the following, we will list the modification to the algorithm for the REAL-SU-SM model.

Instead of optimizing on the expanded network $H$, we now optimize on the multi-arc network $F$. $F$ has the same vertex set as $D$, $V(F) = V(D)$.
Each arc $e \in E(D)$ is mapped into $d(e)$ number of parallel arcs $e_1 \dots e_{d(e)}$ where $d(e)$ is the maximum number of data streams for link $e$. The arcs have non-increasing capacities such that $c(e_k) = c_k(e)$. 

The FD-MTFS algorithm for the MAX-SU-SM model performs maximum weighted matching on the expanded network $H$ iteratively. 
Similarly, the FD-MTFS algorithm for REAL-SU-SM model performs {\em maximum weighted simple $b$-matching}~\cite{Korte12} on the multi-arc network $F$ iteratively.
\begin{mydef}{Maximum Weighted Simple $b$-matching.} Let $G$ be an undirected graph with numbers $b: V(G) \mapsto \mathbb{N}$ and weights $c: E(G) \mapsto \mathbb{R}$, then a {\em simple $b$-matching} in $G$ is a function $f: E(G) \mapsto \{0, 1\}$ and $\sum_{e \in \delta(v)} f(e) \le b(v)$ for all $v \in V(G)$ where $\delta(v)$ is the set of edges incident to $v$. A {\em maximum weighted simple $b$-matching} $f$ is a simple $b$-matching whose weight $\sum_{e \in E(G)} c(e) f(e)$ is maximum.
\end{mydef}

Analogously, the FD-MTFS problem for the REAL-SU-SM model can be mathematically formulated with the help of the {\em node-simple-$b$-matching matrix}.
\begin{mydef}{Node-$b$-matching Matrix.}
	Given a multi-arc network $F$, suppose the number of all possible simple $b$-matching in $F$ is $K$.
	Then the node-$b$-matching matrix $\mat{A} = [a_{i, j}]$ is a $|V(F)| \times K$ matrix. Each element $a_{i, j}$ is equal to the sum capacity of all arcs in the $j$-th simple $b$-matching that enter the $i$-th vertex minus the sum capacity of all arcs in the simple $j$-th $b$-matching that leave the $i$-th vertex.
\end{mydef} 

\begin{figure}[!hbpt]
	\begin{minipage}{0.3\textwidth}
		\begin{figure}[H]
			\includegraphics[width=8cm]{figs/node-b-matching.eps}	
		\end{figure}
	\end{minipage} \\ \\ \\ 
	$\mat{A:}$
	\begin{minipage}{0.7\textwidth} \footnotesize
		$\begin{blockarray}{ccccccccccccccccc}
		& \alpha_1  & \alpha_2  & \beta_1  & \alpha_1,\alpha_2  & \alpha_1, \beta_1  & \alpha_2, \beta_1 \\
		\begin{block}{c[cccccccccccccccc]}
		v_0  & -8 & -6 & 0   & -14 & -8 & -6  \\
		v_1  & 8  & 6  & -3  & 14  & 5  & 3 \\
		v_2  & 0  & 0  & 3   & 0   & 3  & 3  \\
		\end{block}
		\end{blockarray}$
	\end{minipage}
	\caption{Node-$b$-matching matrix $\mat{A}$. $v_0, v_1$ and $v_2$ are the nodes in backhaul network, each with 2 RF chains.
		The maximum number of data streams of each link is $d(\alpha) = 2, d(\beta) = 1$.
		 The arc capacities in the multi-arc network $F$ are: $c(\alpha_1) = 8$, $c(\alpha_2) = 6$, $c(\beta_1) = 3$.}
	\label{fig:node-b-matching}
\end{figure}

Fig.~\ref{fig:node-b-matching} gives an example of the node-$b$-matching matrix. Correspondingly, we define $\mat{A}^M$ as the submatrix of $\mat{A}$ related to the relay BSs in $F$. The set of arcs scheduled in each timeslot must be a simple $b$-matching in $F$. We define $\vect{c}$ as {\em capacity vector} whose element $c_j$ is the cumulative capacity of all macro-BS-to-relay-BS data streams in the $j$-th simple $b$-matching $M_j$, i.e.,
$c_j = \sum_{\{e | e \in M_j, \text{tail}(e) \in B(F) \}} c(e)$ where $B(F)$ are the vertex set of macro-BSs in $F$.
Consequently, the linear program formulation for the FD-MTFS problem for the REAL-SU-SM model is exactly the same as \eqref{eq:mtf-theta} and \eqref{eq:mtf}.
It can be solved in polynomial time by Alg.~\ref{alg:mtf-theta} and \ref{alg:mtf} with slight modification.
Line \ref{alg:mtf-a1} of Alg.~\ref{alg:mtf-theta} is replaced by:

\small
Set weight $w(e_m)$ to each arc $e_m = (v_i, v_j)_m \in E(F)$ where
\begin{equation*}
w(e_m) \eqdef
\begin{cases}
c(e_m) (p_j - p_i) & \text{if }v_i \in M(D)
\\
c(e_m) p_j         & \text{otherwise}.
\end{cases} 
\end{equation*}
Do max weighted simple $b$-matching on $F$ and let the max weight be $z$.  Compute $\eta_1 = -z - p_{\card{M(D)}+1}$
\normalsize

Line \ref{alg:mtf-b1} of Alg.~\ref{alg:mtf} is replaced by:

\small
Set weight $w(e_m)$ to each arc $e_m = (v_i, v_j)_m \in E(F)$ where
\begin{equation*}
w(e_m) \eqdef 
\begin{cases}
c(e_m) (p_j - p_i) & \text{if }v_i \in M(D) \\
c(e_m) (p_j + 1)   & \text{otherwise}.
\end{cases}
\end{equation*}
Do max weighted simple $b$-matching on $F$ and let the max weight be $z$. Compute $\eta_1 = -z - p_{\card{M(D)}+1}$
\normalsize

The initial basic solution to \eqref{eq:mtf-theta} is constructed by replacing $H'$ with $F'$ which is a subgraph of $F$ such that $E(F') = \{e_1 | e \in E(D)\}$. Analogously, the FD-MTFS problem for the REAL-SU-SM model can be solved in polynomial time.
\begin{thm}
	\label{thm:Fd-MTFS-REAL-poly}
	The FD-MTFS problem for the REAL-SU-SM model can be solved in polynomial time with the ellipsoid algorithm.
\end{thm}
